COCO-DR: Combating Distribution Shifts in Zero-Shot Dense Retrieval with Contrastive and Distributionally Robust Learning

We present a new zero-shot dense retrieval (ZeroDR) method, COCO-DR, to improve the generalization ability of dense retrieval by combating the distribution shifts between source training tasks and target scenarios. To mitigate the impact of document differences, COCO-DR continues pretraining the language model on the target corpora to adapt the model to target distributions via COtinuous COtrastive learning. To prepare for unseen target queries, COCO-DR leverages implicit Distributionally Robust Optimization (iDRO) to reweight samples from different source query clusters for improving model robustness over rare queries during fine-tuning. COCO-DR achieves superior average performance on BEIR, the zero-shot retrieval benchmark. At BERT Base scale, COCO-DR Base outperforms other ZeroDR models with 60x larger size. At BERT Large scale, COCO-DR Large outperforms the giant GPT-3 embedding model which has 500x more parameters. Our analysis show the correlation between COCO-DR's effectiveness in combating distribution shifts and improving zero-shot accuracy. Our code and model can be found at \url{https://github.com/OpenMatch/COCO-DR}.

==> Figures/fig_coco.tex <==
\begin{figure}[t]
    % \vspace{-4mm}
    %\begin{small}
        \centering
        \hspace{-2mm}
        \subfigure[COCO loss v.s. BEIR gain]{
    \includegraphics[width=0.5\textwidth]{Figures/BEIR_loss_gain_regplot.pdf}
            \label{fig:coco_gain}
        }\hfill  \hspace{-5mm}
        \subfigure[$\ell_{\text{uniform}}-\ell_{\text{align}}$]{
            \includegraphics[width=0.5\textwidth]{Figures/BEIR_Uniform.pdf}
            \label{fig:uni_align}
        }
        % \vspace{-0ex}
        \caption{
        Left: The relation between the gain of COCO v.s. the gain (both in \%) on BEIR  tasks.
        Right: $\ell_{\text{uniform}}-\ell_{\text{align}}$ plot for {\model} and its variants on BEIR tasks.
        } \label{fig:coco_detail}
        \vspace{-2ex}
    %\end{small}\
\end{figure}

==> Figures/fig_idro.tex <==
\begin{figure}[t]
    % \vspace{-2mm}
    %\begin{small}
        \centering
        % \hspace{-2mm}
        %     \subfigure[iDRO loss v.s. BEIR gain]{
        % \includegraphics[width=0.5\textwidth]{Figures/idro_q_gain.pdf}
        %         \label{fig:coco_gain}
        %     }\hfill  \hspace{-5mm}
        \includegraphics[width=0.6\linewidth]{Figures/idro_q_gain.pdf}

        % \subfigure[$\ell_{\text{uniform}}-\ell_{\text{align}}$]{
        %     \includegraphics[width=0.5\textwidth]{Figures/BEIR_Uniform.pdf}
        %     \label{fig:uni_align}
        % }
        % \vspace{-0ex}
        \caption{
        The relation between the gain on BEIR tasks v.s. the gain on nearest {\marco} groups (in \%). %\cx{add 6b on the performance on these nearest group versus overall MARCO before and after iDRO}
        } \label{fig:idro}
    %\end{small}\
\end{figure}

==> Tables/analysis_bm25.tex <==
\begin{table}[t]
  \small
  \centering
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}l|c|c|c|c|c|c@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & 
% \multicolumn{2}{c|}{Lexical / Sparse}                & 
% \cmidrule(l){2-10} 
\multicolumn{1}{c|}{\multirow{2}{*}{\model}}        & \multicolumn{1}{c|}{\multirow{2}{*}{w/o iDRO}}      & 
\multicolumn{1}{c|}{\multirow{2}{*}{w/o COCO}}      & \multicolumn{1}{c|}{\multirow{2}{1.7cm}{\centering coCondenser \\ (Our Impl.)}}  & \multicolumn{1}{c|}{\centering \multirow{2}{1.9cm}{ coCondenser\\(Official ckpt.)}} &
\multicolumn{1}{c}{\multirow{2}{*}{Condenser}}  \\ 
& & & &  & &\\ \midrule
{\marco}     &
\textbf{0.789} &	0.771 &	0.763 &	0.758 &	0.715 &	0.728 \\
TREC-COVID     &
\textbf{0.789} &	0.771 &	0.763 &	0.758 &	0.715 &	0.728 \\
BioASQ      & 
\textbf{0.429} &	0.424 &	0.353 &	0.341 &	0.318 &	0.330 \\
NFCorpus             & 
\textbf{0.355} &	0.354 &	0.333 &	0.326 &	0.307 &	0.282 \\
NQ          & 
0.505 &	0.503 &	\textbf{0.506} &	0.503 &	0.494 &	0.472 \\
HotpotQA         &
\textbf{0.616} &	0.610 &	0.592 &	0.584 &	0.566 &	0.572 \\
FiQA-2018    & 
0.307 &	0.302 &	\textbf{0.312} &	0.303 &	0.285 &	0.254 \\
Signal-1M          & 
0.271 &	0.275 &	\textbf{0.281} &	0.274 &	0.274 &	0.266 \\
Trec-News               &
0.403 &	0.398 &	\textbf{0.426} &	0.400 &	0.389 &	0.375 \\
Robust04      &
0.443 &	0.443 &	\textbf{0.446} &	0.442 &	0.399 &	0.385 \\
ArguAna          & 
\textbf{0.493} &	0.479 &	0.473 &	0.460 &	0.411 &	0.439 \\
Touché-2020      & 
0.239 &	0.238 &	\textbf{0.257} &	0.243 &	0.190 &	0.236 \\
Quora                & 
0.867 &	\textbf{0.868} &	0.862 &	0.860 &	0.863 &	0.855 \\
DBPedia-entity              & 
\textbf{0.391} &	0.389 &	0.382 &	0.364 &	0.356 &	0.362 \\
SCIDOCS            & 
0.160 &	\textbf{0.161} &	0.154 &	0.150 &	0.140 &	0.143 \\
Fever            & 
0.751 &	\textbf{0.757} &	0.739 &	0.751 &	0.678 &	0.725 \\
Climate-Fever         & 
\textbf{0.211} &	0.209 &	0.202 &	0.208 &	0.184 &	0.206 \\
SciFact               & 
\textbf{0.709} &	0.688 &	0.615 &	0.602 &	0.600 &	0.581 \\
CQADupStack         & 
\textbf{0.370} &	0.365 &	0.349 &	0.342 &	0.330 &	0.313 \\ \midrule
Avg           & 
\textbf{0.462} &	0.457 &	0.447 &	0.440 &	0.417 &	0.418 \\
% Avg w/o MS Marco                                      & \multicolumn{1}{c|}{0.423}          & {\underline{0.434}}    & \multicolumn{1}{c|}{0.237} & \multicolumn{1}{c|}{0.389} & \multicolumn{1}{c|}{{\underline{0.415}}} & \multicolumn{1}{c|}{0.410} & 0.431          & \multicolumn{1}{c|}{0.416}    & \multicolumn{1}{c|}{0.445}     & \multicolumn{1}{c|}{0.453}          & \textbf{0.458} \\ 
\bottomrule
\end{tabular}
  }
  \caption{NDCG@10 on the BEIR benchmark. The best result on a given dataset is marked in bold. GTR models are pre-trained on CommunityQA dataset and the complete MS Marco dataset. GTR models achieve better NDCG when increasing size from Base to XXL, outperforming the previous best sparse model DocT5Query and dense retrieval model TAS-B. 
  $^\dagger$: Train an independent model for each task.\
  $^\ddagger$: Larger Model (Billion-scale), more training data (CommunityQA or code-text pairs).  \ 
  $^\#$: Require a reranker.
  Single model/vector, dense retrieval
  \yue{Copy from GTR paper, add GPL, Laprador, CPT, Contriever, Modir?}
  \cx{mark one difference of coCondense is the usage of RocketQA added title which is a web search unique property.}
  }
  \label{tab:abla_ndcg}
\end{table}

==> Tables/main_abla_large.tex <==
\begin{table}[t]
%   \small
% \vspace{-1.5ex}
  \centering
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{l|ccc|c|c}
\toprule
Method ($\rightarrow$) & \multicolumn{3}{c|}{COCO-DR Large}      & {coCondenser}   &
Condenser  \\ 
Dataset ($\downarrow$) & Full & -iDRO & -COCO & Ours &  Ours \\ \hline
TREC-COVID     &
\bf 0.804&	0.797&	0.745&	0.745&	0.780 \\
BioASQ      & 
0.449&\bf 	0.450&	0.413&	0.410&	0.381
 \\
NFCorpus             & 
\bf 0.354&	0.353&	0.349&	0.350&	0.317
\\
NQ          & 
\bf 0.547&	0.536&	0.519&	0.516&	0.492 \\
HotpotQA         &
0.641&\bf 	0.644&	0.614&	0.616&	0.591 \\
FiQA-2018    &\bf  0.329&	0.322&	0.328&	0.326	&0.280 \\
Signal-1M          & 0.285&	0.285	&\bf 0.296	&0.295&	0.284 \\
TREC-NEWS               & \bf 0.432	&0.426&	0.413&	0.416&	0.423 \\
Robust04      & \bf 0.482&	0.467&	0.466&	0.461&	0.418 \\
ArguAna          &  \bf 0.515&	0.513&	0.488&	0.484&	0.469 \\
Touché-2020      & 
\bf 0.263	&0.258	&0.249&	0.246&	0.244 \\
Quora                & 
\bf 0.872&	0.869&	0.865&	0.862&	0.852 \\
DBPedia-entity              & 
\bf 0.407&	0.401&	0.388&	0.386&	0.364\\
SCIDOCS            & 
\bf 0.178&	0.176&	0.171&	0.171&	0.161\\
Fever            & 
\bf 0.793&	0.783&	0.741&	0.724&	0.736 \\
Climate-Fever         & 
\bf 0.247&	0.240&	0.233&	0.226&	0.216 \\
SciFact               & 
\bf 0.722&	0.709&	0.696&	0.686&	0.661 \\
CQADupStack         & \bf 0.393	&0.385	&0.367&	0.363&	0.343 \\\hline
Avg           & 
\bf 0.484&	0.478 &	0.463 &	0.460 &	0.445\\
% Avg w/o MS Marco                                      & \multicolumn{1}{c|}{0.423}          & {\underline{0.434}}    & \multicolumn{1}{c|}{0.237} & \multicolumn{1}{c|}{0.389} & \multicolumn{1}{c|}{{\underline{0.415}}} & \multicolumn{1}{c|}{0.410} & 0.431          & \multicolumn{1}{c|}{0.416}    & \multicolumn{1}{c|}{0.445}     & \multicolumn{1}{c|}{0.453}          & \textbf{0.458} \\ 
\bottomrule
\end{tabular}
  }
  \caption{Ablation study of \model{} with BERT-Large as the backbone.
%   The results of ``-COCO” only pretrain and finetune on {\marco}, similar to {\cocondenser}. 
%   A key difference is the use of MARCO title in \citet{cocondenser} which hurts zero-shot performance.
  }
%   \vspace{-1ex}
  \label{tab:abla_large}
\end{table}





==> Tables/main_exp_full.tex <==
\begin{table*}[t]
  \small
  \centering
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}l|cc|ccccccccccccc|c@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Datasets}} & \multicolumn{2}{c|}{Lexical / Sparse}                & \multicolumn{12}{c|}{Dense}    & \multicolumn{1}{c|}{Late-Interaction}           & \multicolumn{1}{c}{Ours}                                                                                              \\ \cmidrule(l){2-17} 
\multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{BM25}           & docT5query$^\dagger$     & \multicolumn{1}{c|}{DPR}   & \multicolumn{1}{c|}{ANCE}  & \multicolumn{1}{c|}{TAS-B$^\#$}       & \multicolumn{1}{c|}{LaPraDor}  & \multicolumn{1}{c|}{Contriver} &
\multicolumn{1}{c|}{GenQ$^\dagger$} & \multicolumn{1}{c|}{MoDIR$^\dagger$} & \multicolumn{1}{c|}{GPL$^{\dagger,\#}$} &
\multicolumn{1}{c|}{CPT{\tiny{L}}$^\ddagger$}  & \multicolumn{1}{c|}{CPT{\tiny{XL}}$^\ddagger$} &  
% \multicolumn{1}{c|}{GTR\tiny{Base}} & \multicolumn{1}{c|}{GTR\tiny{Large}} &
\multicolumn{1}{c|}{GTR{\tiny{XL}}$^\ddagger$}         & \multicolumn{1}{c|}{GTR{\tiny{XXL}}$^\ddagger$}   &\multicolumn{1}{c|}{ColBERT}        &  \multicolumn{1}{c}{\ours}     \\ \midrule
MS Marco                                              & \multicolumn{1}{c|}{0.228}          & 0.338          & \multicolumn{1}{c|}{0.177} & \multicolumn{1}{c|}{0.388} & \multicolumn{1}{c|}{0.408}    & \multicolumn{1}{c|}{0.366} & \multicolumn{1}{c|}{0.407} & \multicolumn{1}{c|}{0.408} 
& \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{---}
   & \multicolumn{1}{c|}{0.439}          & \multicolumn{1}{c|}{0.442}  & \multicolumn{1}{c|}{0.401}        & {0.419} \\
\midrule
Trec-Covid                                            & \multicolumn{1}{c|}{0.656}          & \textbf{0.713} & \multicolumn{1}{c|}{0.332} & \multicolumn{1}{c|}{0.654}
& \multicolumn{1}{c|}{0.481}       
&  \multicolumn{1}{c|}{0.492} & \multicolumn{1}{c|}{0.596} & \multicolumn{1}{c|}{0.619} & \multicolumn{1}{c|}{0.676}  & \multicolumn{1}{c|}{0.700} & \multicolumn{1}{c|}{0.642} & \multicolumn{1}{c|}{0.649} & \multicolumn{1}{c|}{0.584} & \multicolumn{1}{c|}{0.501} & \multicolumn{1}{c|}{0.677}  & {0.788}     \\
BioASQ                                                & \multicolumn{1}{c|}{0.465}          & 0.431          & \multicolumn{1}{c|}{0.127} & \multicolumn{1}{c|}{0.306} & \multicolumn{1}{c|}{0.383}       
& \multicolumn{1}{c|}{0.308} &    \multicolumn{1}{c|}{---}     
& \multicolumn{1}{c|}{0.398} 
& \multicolumn{1}{c|}{0.320} &    \multicolumn{1}{c|}{0.442}
& \multicolumn{1}{c|}{---} &    \multicolumn{1}{c|}{---}
& \multicolumn{1}{c|}{0.317}          & 0.324    & \textbf{0.474}  & {0.425}  \\
NFCorpus              & \multicolumn{1}{c|}{0.325}          & 0.328          & \multicolumn{1}{c|}{0.189} & \multicolumn{1}{c|}{0.237} & \multicolumn{1}{c|}{0.319}       
& \multicolumn{1}{c|}{0.335} & \multicolumn{1}{c|}{0.328}   
& \multicolumn{1}{c|}{0.319} & \multicolumn{1}{c|}{0.244}  & \multicolumn{1}{c|}{0.345} & \multicolumn{1}{c|}{0.380}& \multicolumn{1}{c|}{0.407}    & \multicolumn{1}{c|}{\textbf{0.343}} & \multicolumn{1}{c|}{0.342} & \multicolumn{1}{c|}{0.305} & 0.356         \\
NQ          & \multicolumn{1}{c|}{0.329}          & 0.399          & \multicolumn{1}{c|}{0.474}  & \multicolumn{1}{c|}{0.446} & \multicolumn{1}{c|}{0.463}  
& \multicolumn{1}{c|}{0.473} & \multicolumn{1}{c|}{0.498}  
& \multicolumn{1}{c|}{0.358} & 0.524             
& \multicolumn{1}{c|}{0.559}          & \textbf{0.568} \\
HotpotQA                                              & \multicolumn{1}{c|}{\textbf{0.603}} & 0.58           & \multicolumn{1}{c|}{0.391} & \multicolumn{1}{c|}{0.456} & \multicolumn{1}{c|}{0.584}       & \multicolumn{1}{c|}{0.534} & 0.593          & \multicolumn{1}{c|}{0.535}    & \multicolumn{1}{c|}{0.579}     & \multicolumn{1}{c|}{0.591}          & 0.599          \\
FiQA-2018                                             & \multicolumn{1}{c|}{0.236}          & 0.291          & \multicolumn{1}{c|}{0.112} & \multicolumn{1}{c|}{0.295} & \multicolumn{1}{c|}{0.300}       & \multicolumn{1}{c|}{0.308} & 0.317          & \multicolumn{1}{c|}{0.349}    & \multicolumn{1}{c|}{0.424}     & \multicolumn{1}{c|}{0.444}          & \textbf{0.467} \\
Signal-1M                                             & \multicolumn{1}{c|}{\textbf{0.330}} & 0.307          & \multicolumn{1}{c|}{0.155} & \multicolumn{1}{c|}{0.249} & \multicolumn{1}{c|}{0.289}       & \multicolumn{1}{c|}{0.281} & 0.274          & \multicolumn{1}{c|}{0.261}    & \multicolumn{1}{c|}{0.265}     & \multicolumn{1}{c|}{0.268}          & 0.273          \\
TREC-NEWS                                             & \multicolumn{1}{c|}{0.398}          & \textbf{0.42}  & \multicolumn{1}{c|}{0.161} & \multicolumn{1}{c|}{0.382} & \multicolumn{1}{c|}{0.377}       & \multicolumn{1}{c|}{0.396} & 0.393          & \multicolumn{1}{c|}{0.337}    & \multicolumn{1}{c|}{0.343}     & \multicolumn{1}{c|}{0.350}          & 0.346          \\
Robust04                                              & \multicolumn{1}{c|}{0.408}          & 0.437          & \multicolumn{1}{c|}{0.252} & \multicolumn{1}{c|}{0.392} & \multicolumn{1}{c|}{0.427}       & \multicolumn{1}{c|}{0.362} & 0.391          & \multicolumn{1}{c|}{0.437}    & \multicolumn{1}{c|}{0.470}     & \multicolumn{1}{c|}{0.479}          & \textbf{0.506} \\
ArguAna                                               & \multicolumn{1}{c|}{0.315}          & 0.349          & \multicolumn{1}{c|}{0.175} & \multicolumn{1}{c|}{0.415} & \multicolumn{1}{c|}{0.429}       & \multicolumn{1}{c|}{0.493} & 0.233          & \multicolumn{1}{c|}{0.511}    & \multicolumn{1}{c|}{0.525}     & \multicolumn{1}{c|}{0.531}          & \textbf{0.540} \\
Touché-2020                                           & \multicolumn{1}{c|}{\textbf{0.367}} & 0.347          & \multicolumn{1}{c|}{0.131} & \multicolumn{1}{c|}{0.240} & \multicolumn{1}{c|}{0.162}       & \multicolumn{1}{c|}{0.182} & 0.202          & \multicolumn{1}{c|}{0.205}    & \multicolumn{1}{c|}{0.219}     & \multicolumn{1}{c|}{0.230}          & 0.256          \\
Quora                                                 & \multicolumn{1}{c|}{0.789}          & 0.802          & \multicolumn{1}{c|}{0.248} & \multicolumn{1}{c|}{0.852} & \multicolumn{1}{c|}{0.835}       & \multicolumn{1}{c|}{0.830} & 0.854          & \multicolumn{1}{c|}{0.881}    & \multicolumn{1}{c|}{0.890}     & \multicolumn{1}{c|}{0.890}          & \textbf{0.892} \\
DBPedia-entity                                        & \multicolumn{1}{c|}{0.313}          & 0.331          & \multicolumn{1}{c|}{0.263} & \multicolumn{1}{c|}{0.281} & \multicolumn{1}{c|}{0.384}       & \multicolumn{1}{c|}{0.328} & 0.392          & \multicolumn{1}{c|}{0.347}    & \multicolumn{1}{c|}{0.391}     & \multicolumn{1}{c|}{0.396}          & \textbf{0.408} \\
SCIDOCS                                               & \multicolumn{1}{c|}{0.158}          & \textbf{0.162} & \multicolumn{1}{c|}{0.077} & \multicolumn{1}{c|}{0.122} & \multicolumn{1}{c|}{0.149}       & \multicolumn{1}{c|}{0.143} & 0.145          & \multicolumn{1}{c|}{0.149}    & \multicolumn{1}{c|}{0.158}     & \multicolumn{1}{c|}{0.159}          & 0.161          \\
Fever                                                 & \multicolumn{1}{c|}{0.753}          & 0.714          & \multicolumn{1}{c|}{0.562} & \multicolumn{1}{c|}{0.669} & \multicolumn{1}{c|}{0.700}       & \multicolumn{1}{c|}{0.669} & \textbf{0.771} & \multicolumn{1}{c|}{0.660}    & \multicolumn{1}{c|}{0.712}     & \multicolumn{1}{c|}{0.717}          & 0.740          \\
Climate-Fever                                         & \multicolumn{1}{c|}{0.213}          & 0.201          & \multicolumn{1}{c|}{0.148} & \multicolumn{1}{c|}{0.198} & \multicolumn{1}{c|}{0.228}       & \multicolumn{1}{c|}{0.175} & 0.184          & \multicolumn{1}{c|}{0.241}    & \multicolumn{1}{c|}{0.262}     & \multicolumn{1}{c|}{\textbf{0.270}} & 0.267          \\
SciFact                                               & \multicolumn{1}{c|}{0.665}          & \textbf{0.675} & \multicolumn{1}{c|}{0.318} & \multicolumn{1}{c|}{0.507} & \multicolumn{1}{c|}{0.643}       & \multicolumn{1}{c|}{0.644} & 0.671          & \multicolumn{1}{c|}{0.600}    & \multicolumn{1}{c|}{0.639}     & \multicolumn{1}{c|}{0.635}          & 0.662          \\
CQADupStack                                           & \multicolumn{1}{c|}{0.299}          & 0.325          & \multicolumn{1}{c|}{0.153} & \multicolumn{1}{c|}{0.296} & \multicolumn{1}{c|}{0.314}       & \multicolumn{1}{c|}{0.347} & 0.350          & \multicolumn{1}{c|}{0.357}    & \multicolumn{1}{c|}{0.384}     & \multicolumn{1}{c|}{0.388}          & \textbf{0.399} \\ \midrule
Avg_{\text{11}}                                                   & \multicolumn{1}{c|}{0.413}          & 0.429          & \multicolumn{1}{c|}{0.234} & \multicolumn{1}{c|}{0.389} & \multicolumn{1}{c|}{0.414}       & \multicolumn{1}{c|}{0.410} & 0.429          & \multicolumn{1}{c|}{0.416}    & \multicolumn{1}{c|}{0.444}     & \multicolumn{1}{c|}{0.452}          & \textbf{0.457} \\
Avg                                                   & \multicolumn{1}{c|}{0.413}          & 0.429          & \multicolumn{1}{c|}{0.234} & \multicolumn{1}{c|}{0.389} & \multicolumn{1}{c|}{0.414}       & \multicolumn{1}{c|}{0.410} & 0.429          & \multicolumn{1}{c|}{0.416}    & \multicolumn{1}{c|}{0.444}     & \multicolumn{1}{c|}{0.452}          & \textbf{0.457} \\
% Avg w/o MS Marco                                      & \multicolumn{1}{c|}{0.423}          & {\underline{0.434}}    & \multicolumn{1}{c|}{0.237} & \multicolumn{1}{c|}{0.389} & \multicolumn{1}{c|}{{\underline{0.415}}} & \multicolumn{1}{c|}{0.410} & 0.431          & \multicolumn{1}{c|}{0.416}    & \multicolumn{1}{c|}{0.445}     & \multicolumn{1}{c|}{0.453}          & \textbf{0.458} \\ 
\bottomrule
\end{tabular}
  }
  \caption{NDCG@10 on the BEIR benchmark. The best result on a given dataset is marked in bold. GTR models are pre-trained on CommunityQA dataset and the complete MS Marco dataset. GTR models achieve better NDCG when increasing size from Base to XXL, outperforming the previous best sparse model DocT5Query and dense retrieval model TAS-B. 
  $^\dagger$: Train an independent model for each task.\
  $^\ddagger$: Larger Model (Billion-scale), more training data (CommunityQA or code-text pairs).  \ 
  $^\#$: Require a reranker.
  Single model/vector, dense retrieval
  \yue{Copy from GTR paper, add GPL, Laprador, CPT, Contriever, Modir?}}
  \label{tab:all_ndcg}
\end{table*}

==> Tables/main_exp_gtr.tex <==
\begin{table*}[t]
  \small
  \centering
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}l|c|ccccccccccc|cc@{}}
\toprule
\multicolumn{1}{c|}{{\textbf{Method} ($\rightarrow$)}} & \multicolumn{1}{c|}{\textbf{Sparse}}                & \multicolumn{10}{c|}{\textbf{Dense}}    & \multicolumn{1}{c|}{\textbf{Late-Inter.}}           & \multicolumn{2}{c}{\textbf{\model{} (Ours)}}     \\  \cmidrule(l){2-15} 
\multicolumn{1}{c|}{\textbf{Dataset} ($\downarrow$)}          & \multicolumn{1}{c|}{BM25}
% & docT5query$^\dagger$     
& \multicolumn{1}{c|}{DPR}   & \multicolumn{1}{c|}{ANCE}  
% \multicolumn{1}{c|}{TAS-B$^\#$}      
& \multicolumn{1}{c|}{LaPraDor}  & \multicolumn{1}{c|}{Contriver} &
\multicolumn{1}{c|}{GenQ$^\dagger$} 
% & \multicolumn{1}{c|}{MoDIR$^\dagger$} 
& \multicolumn{1}{c|}{GPL$^{\dagger,\#}$} &
\multicolumn{1}{c|}{CPT{\tiny{L}}$^\ddagger$}  & \multicolumn{1}{c|}{CPT{\tiny{XL}}$^\ddagger$} &  
% \multicolumn{1}{c|}{GTR\tiny{Base}} & \multicolumn{1}{c|}{GTR\tiny{Large}} &
\multicolumn{1}{c|}{GTR{\tiny{XL}}$^\ddagger$}         & \multicolumn{1}{c|}{GTR{\tiny{XXL}}$^\ddagger$}   &\multicolumn{1}{c|}{ColBERT}        &  \multicolumn{1}{c|}{\text{Base}} & \multicolumn{1}{c}{\text{Large}}     \\ \midrule
MS Marco                                              & \multicolumn{1}{c|}{0.228}         % & 0.338          
& \multicolumn{1}{c|}{0.354} & \multicolumn{1}{c|}{0.388}     & \multicolumn{1}{c|}{0.366} & \multicolumn{1}{c|}{0.407} & \multicolumn{1}{c|}{0.408} 
& \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{---}
   & \multicolumn{1}{c|}{0.439}          & \multicolumn{1}{c|}{0.442}  & \multicolumn{1}{c|}{0.401}        & \multicolumn{1}{c|}{0.419} & {0.424} \\
\midrule
TREC-COVID                                           & \multicolumn{1}{c|}{0.656}          %& \textbf{0.713} 
& \multicolumn{1}{c|}{0.575} & \multicolumn{1}{c|}{0.654}
% & \multicolumn{1}{c|}{0.481}       
&  \multicolumn{1}{c|}{0.492} & \multicolumn{1}{c|}{0.596} & \multicolumn{1}{c|}{0.619} &  \multicolumn{1}{c|}{0.700} & \multicolumn{1}{c|}{0.642} & \multicolumn{1}{c|}{0.649} & \multicolumn{1}{c|}{0.584} & \multicolumn{1}{c|}{0.501} & \multicolumn{1}{c|}{0.677}  & \multicolumn{1}{c|}{{0.789}} &    \textbf{0.804}  \\
BioASQ                                                & \multicolumn{1}{c|}{0.465}          
%& 0.431          
& \multicolumn{1}{c|}{0.232} & \multicolumn{1}{c|}{0.306} 
% & \multicolumn{1}{c|}{0.383}       
& \multicolumn{1}{c|}{0.308} &    \multicolumn{1}{c|}{---}     
& \multicolumn{1}{c|}{0.398} &    \multicolumn{1}{c|}{0.442}
& \multicolumn{1}{c|}{---} &    \multicolumn{1}{c|}{---}
& \multicolumn{1}{c|}{0.317}          & \multicolumn{1}{c|}{0.324}    & \textbf{0.474}  & \multicolumn{1}{c|}{0.429} & {0.449}  \\
NFCorpus              & \multicolumn{1}{c|}{0.325}          %& 0.328        
& \multicolumn{1}{c|}{0.210} & \multicolumn{1}{c|}{0.237} 
% & \multicolumn{1}{c|}{0.319}       
& \multicolumn{1}{c|}{0.335} & \multicolumn{1}{c|}{0.328}   
& \multicolumn{1}{c|}{0.319} & \multicolumn{1}{c|}{0.345} & \multicolumn{1}{c|}{0.380}& \multicolumn{1}{c|}{\textbf{0.407}}    & \multicolumn{1}{c|}{0.343} & \multicolumn{1}{c|}{0.342} & \multicolumn{1}{c|}{0.305} & \multicolumn{1}{c|}{0.355} & 0.354         \\
NQ          & \multicolumn{1}{c|}{0.329}          & \multicolumn{1}{c|}{0.398}          & \multicolumn{1}{c|}{0.446}  & \multicolumn{1}{c|}{0.473} & \multicolumn{1}{c|}{0.498}  
& \multicolumn{1}{c|}{0.358} & \multicolumn{1}{c|}{0.483}  
& \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{---}             
& \multicolumn{1}{c|}{0.559$^*$}          & \multicolumn{1}{c|}{\textbf{0.568}$^*$}
& \multicolumn{1}{c|}{0.524} & \multicolumn{1}{c|}{0.505} & \textbf{0.547} \\
HotpotQA                       & \multicolumn{1}{c|}{0.603} & \multicolumn{1}{c|}{0.371}           & \multicolumn{1}{c|}{0.456} & \multicolumn{1}{c|}{0.495} & \multicolumn{1}{c|}{0.638}       & \multicolumn{1}{c|}{0.534} & \multicolumn{1}{c|}{0.582}          & \multicolumn{1}{c|}{0.648}    & \multicolumn{1}{c|}{\textbf{0.688}}     & \multicolumn{1}{c|}{0.591}          & \multicolumn{1}{c|}{0.599} & 0.593 & \multicolumn{1}{c|}{0.616}  &  0.641       \\
FiQA-2018                                             & \multicolumn{1}{c|}{0.236}          & \multicolumn{1}{c|}{0.274}          & \multicolumn{1}{c|}{0.295} & \multicolumn{1}{c|}{0.314} & \multicolumn{1}{c|}{0.329}       & \multicolumn{1}{c|}{0.308} & \multicolumn{1}{c|}{0.344}          & \multicolumn{1}{c|}{0.452}    & \multicolumn{1}{c|}{\textbf{0.512}}     & \multicolumn{1}{c|}{0.444}          & \multicolumn{1}{c|}{0.467} & 0.317 & \multicolumn{1}{c|}{0.307} & 0.329 \\
Signal-1M                                             & \multicolumn{1}{c|}{\textbf{0.330}} & \multicolumn{1}{c|}{0.238}          & \multicolumn{1}{c|}{0.249} & \multicolumn{1}{c|}{0.231} & \multicolumn{1}{c|}{---}       & \multicolumn{1}{c|}{0.281} & \multicolumn{1}{c|}{0.276}          & \multicolumn{1}{c|}{---}    & \multicolumn{1}{c|}{---}     & \multicolumn{1}{c|}{0.268}          & \multicolumn{1}{c|}{0.273}   & 0.274 & \multicolumn{1}{c|}{0.271} & 0.285       \\
TREC-NEWS                                             & \multicolumn{1}{c|}{0.398}          & \multicolumn{1}{c|}{0.366}  & \multicolumn{1}{c|}{0.382} & \multicolumn{1}{c|}{0.374} & \multicolumn{1}{c|}{---}       & \multicolumn{1}{c|}{0.396} & \multicolumn{1}{c|}{{0.421}}          & \multicolumn{1}{c|}{---}    & \multicolumn{1}{c|}{---}     & \multicolumn{1}{c|}{0.350}          & \multicolumn{1}{c|}{0.346}   & 0.393 & \multicolumn{1}{c|}{0.403} & \textbf{0.432}       \\
Robust04                                              & \multicolumn{1}{c|}{0.408}          & \multicolumn{1}{c|}{0.344}          & \multicolumn{1}{c|}{0.392} & \multicolumn{1}{c|}{0.368} & \multicolumn{1}{c|}{---}       & \multicolumn{1}{c|}{0.362} & \multicolumn{1}{c|}{0.437}          & \multicolumn{1}{c|}{---}    & \multicolumn{1}{c|}{---}     & \multicolumn{1}{c|}{0.479}          & \multicolumn{1}{c|}{\textbf{0.506}} & 0.391 & \multicolumn{1}{c|}{0.443} & {0.482} \\
ArguAna                                               & \multicolumn{1}{c|}{0.414}          & \multicolumn{1}{c|}{0.414}          & \multicolumn{1}{c|}{0.415} & \multicolumn{1}{c|}{0.469} & \multicolumn{1}{c|}{0.446}       & \multicolumn{1}{c|}{0.493} & \multicolumn{1}{c|}{\textbf{0.557}}          & \multicolumn{1}{c|}{0.469}    & \multicolumn{1}{c|}{0.435}     & \multicolumn{1}{c|}{0.531}          & \multicolumn{1}{c|}{0.540} & 0.233 & \multicolumn{1}{c|}{0.493} & 0.515 \\
Touché-2020                                           & \multicolumn{1}{c|}{\textbf{0.367}} & \multicolumn{1}{c|}{0.208}          & \multicolumn{1}{c|}{0.240} & \multicolumn{1}{c|}{0.182} & \multicolumn{1}{c|}{0.230}       & \multicolumn{1}{c|}{0.182} & \multicolumn{1}{c|}{0.255}          & \multicolumn{1}{c|}{0.309}    & \multicolumn{1}{c|}{0.291}     & \multicolumn{1}{c|}{0.230}          & \multicolumn{1}{c|}{0.256} & 0.202 & \multicolumn{1}{c|}{0.239} & 0.263         \\
Quora                                                 & \multicolumn{1}{c|}{0.789}          & \multicolumn{1}{c|}{0.842}          & \multicolumn{1}{c|}{0.852} & \multicolumn{1}{c|}{0.847} & \multicolumn{1}{c|}{0.865}       & \multicolumn{1}{c|}{0.830} & \multicolumn{1}{c|}{0.836}          & \multicolumn{1}{c|}{0.677}    & \multicolumn{1}{c|}{0.638}     & \multicolumn{1}{c|}{0.890}          & \multicolumn{1}{c|}{\textbf{0.892}} & 0.854 & \multicolumn{1}{c|}{0.867} & 0.872\\
DBPedia-entity                                        & \multicolumn{1}{c|}{0.313}          & \multicolumn{1}{c|}{0.236}          & \multicolumn{1}{c|}{0.281} & \multicolumn{1}{c|}{0.338} & \multicolumn{1}{c|}{0.413}       & \multicolumn{1}{c|}{0.328} & \multicolumn{1}{c|}{0.384}          & \multicolumn{1}{c|}{0.412}    & \multicolumn{1}{c|}{\textbf{0.432}}     & \multicolumn{1}{c|}{0.396}          & \multicolumn{1}{c|}{0.408} & 0.392 & \multicolumn{1}{c|}{0.391} & 0.407 \\
SCIDOCS                                               & \multicolumn{1}{c|}{0.158}          & \multicolumn{1}{c|}{0.107} & \multicolumn{1}{c|}{0.122} & \multicolumn{1}{c|}{0.155} & \multicolumn{1}{c|}{0.165}       & \multicolumn{1}{c|}{0.143} & \multicolumn{1}{c|}{{0.169}}          & \multicolumn{1}{c|}{---}    & \multicolumn{1}{c|}{---}     & \multicolumn{1}{c|}{0.159}          & \multicolumn{1}{c|}{0.161}   & 0.145 & \multicolumn{1}{c|}{0.160} & \textbf{0.178}       \\
Fever                                                 & \multicolumn{1}{c|}{0.753}          & \multicolumn{1}{c|}{0.589}          & \multicolumn{1}{c|}{0.669} & \multicolumn{1}{c|}{0.646} & \multicolumn{1}{c|}{0.758}       & \multicolumn{1}{c|}{0.669} & \multicolumn{1}{c|}{0.759} & \multicolumn{1}{c|}{0.756}    & \multicolumn{1}{c|}{{0.775}}     & \multicolumn{1}{c|}{0.717}          & \multicolumn{1}{c|}{0.740}  & 0.771 & \multicolumn{1}{c|}{0.751}   & \textbf{0.793}      \\
Climate-Fever                                         & \multicolumn{1}{c|}{0.213}          & \multicolumn{1}{c|}{0.176}          & \multicolumn{1}{c|}{0.198} & \multicolumn{1}{c|}{0.209} & \multicolumn{1}{c|}{0.237}       & \multicolumn{1}{c|}{0.175} & \multicolumn{1}{c|}{0.235}          & \multicolumn{1}{c|}{0.194}    & \multicolumn{1}{c|}{0.223}     & \multicolumn{1}{c|}{\textbf{0.270}} & \multicolumn{1}{c|}{0.267} & 0.184 & \multicolumn{1}{c|}{0.211}   & 0.247      \\
SciFact                                               & \multicolumn{1}{c|}{0.665}          & \multicolumn{1}{c|}{0.475} & \multicolumn{1}{c|}{0.507} & \multicolumn{1}{c|}{0.599} & \multicolumn{1}{c|}{0.677}       & \multicolumn{1}{c|}{0.644} & \multicolumn{1}{c|}{0.674}          & \multicolumn{1}{c|}{0.744}    & \multicolumn{1}{c|}{\textbf{0.754}}     & \multicolumn{1}{c|}{0.635}          & \multicolumn{1}{c|}{0.662}  & 0.671 & \multicolumn{1}{c|}{0.709}  & 0.722      \\
CQADupStack                                           & \multicolumn{1}{c|}{0.299}          & \multicolumn{1}{c|}{0.281}          & \multicolumn{1}{c|}{0.296} & \multicolumn{1}{c|}{0.288} & \multicolumn{1}{c|}{0.345}       & \multicolumn{1}{c|}{0.347} & \multicolumn{1}{c|}{0.357}          & \multicolumn{1}{c|}{---}    & \multicolumn{1}{c|}{---}     & \multicolumn{1}{c|}{0.388}          & \multicolumn{1}{c|}{\textbf{0.399}} & 0.350 & \multicolumn{1}{c|}{0.370} & 0.393 \\ \midrule
Avg  CPT Sub                                                  & \multicolumn{1}{c|}{0.484}          & \multicolumn{1}{c|}{0.397}          & \multicolumn{1}{c|}{0.437} & \multicolumn{1}{c|}{0.448} & \multicolumn{1}{c|}{0.502}       & \multicolumn{1}{c|}{0.464} & \multicolumn{1}{c|}{0.516}          & \multicolumn{1}{c|}{0.517}    & \multicolumn{1}{c|}{{0.528}}     & \multicolumn{1}{c|}{0.511}          & \multicolumn{1}{c|}{0.516} & 0.473 & \multicolumn{1}{c|}{0.521} & \textbf{0.541}\\
Avg                                                   & \multicolumn{1}{c|}{0.428}          & \multicolumn{1}{c|}{0.352}          & \multicolumn{1}{c|}{0.389} & \multicolumn{1}{c|}{0.396} & \multicolumn{1}{c|}{---}       & \multicolumn{1}{c|}{0.410} & \multicolumn{1}{c|}{0.459}          & \multicolumn{1}{c|}{---}    & \multicolumn{1}{c|}{---}     & \multicolumn{1}{c|}{0.453}          & \multicolumn{1}{c|}{0.458} & 0.431 & \multicolumn{1}{c|}{0.462}& \textbf{0.484} \\
% Avg w/o MS Marco                                      & \multicolumn{1}{c|}{0.423}          & {\underline{0.434}}    & \multicolumn{1}{c|}{0.237} & \multicolumn{1}{c|}{0.389} & \multicolumn{1}{c|}{{\underline{0.415}}} & \multicolumn{1}{c|}{0.410} & 0.431          & \multicolumn{1}{c|}{0.416}    & \multicolumn{1}{c|}{0.445}     & \multicolumn{1}{c|}{0.453}          & \textbf{0.458} \\ 
\bottomrule
\end{tabular}
  }
  \vspace{-1ex}
  \caption{NDCG@10 on the BEIR benchmark. The best result each task is marked bold. Avg CPT Sub stands for the average performance on 11 BEIR tasks used in \citet{cpt}.
%   {\model} outperforms all baselines on the average nDCG over 18 datasets and achieves comparable performance with CPT{\tiny{XL}} which has 1600x more parameters.  
 $^*$: Unfair comparison, NQ is used in training for GTR. 
 $\dagger$: Use generated pseudo labels to train an independent model for each task.\
  $\ddagger$: Larger Model (Billion-scale), more training data (CommunityQA or web-scale internet data).   
  $\#$: Use cross-encoders reranking teachers.}
  \vspace{-1ex}
%   Single model/vector, dense retrieval}
%   \yue{Copy from GTR paper, add GPL, Laprador, CPT, Contriever, Modir?}}
  \label{tab:all_ndcg}
\end{table*}
% \vspace{-1ex}

==> Tables/modir_res.tex <==
\begin{table*}[t]
	\centering
	\small
% 	\resizebox{\textwidth}{!}{
    \begin{tabular}{@{}l|ccc|ccccl@{}}
    \hline
	              & \multicolumn{3}{c|}{\textbf{Hole@10}} & \multicolumn{5}{c}{\textbf{nDCG@10}} \\
                   & BM25 & DPR & ANCE & BM25 &  
                   DPR 
                  & DPR+\model & ANCE & ANCE+\model \\
	 \hline
	 TREC-COVID  & 10.6\% & 33.0\% & 22.4\% & 0.616 & 0.561 & 0.591($+$5.3\%) & 0.654 & 0.676 ($+$3.4\%) \\
	 Touch\'e    & 29.8\% & 63.3\% & 56.9\% & 0.605 & 0.243 & 0.258($+$6.2\%) & 0.284 & 0.315 ($+$10.9\%) \\
	 DBPedia     & 41.3\% & 73.2\% & 65.8\% & 0.288 & 0.236 & 0.240($+$1.7\%) & 0.281 & 0.284 ($+$1.1\%) \\
	 NFCorpus    & 74.1\% & 85.2\% & 83.1\% & 0.297 & 0.208 & 0.212($+$1.9\%) & 0.237 & 0.244 ($+$3.0\%) \\
	 Quora       & 88.7\% & 87.3\% & 87.1\% & 0.742 & 0.842 & 0.848($+$0.7\%) & 0.852 & 0.856 ($+$0.5\%) \\
	 BioASQ      & 80.7\% & 92.0\% & 89.5\% & 0.514 & 0.232 & 0.247($+$6.5\%) & 0.306 & 0.320 ($+$4.6\%) \\
	 HotpotQA    & 87.7\% & 92.3\% & 90.9\% & 0.601 & 0.371 & 0.387($+$4.3\%) & 0.456 & 0.462 ($+$1.3\%) \\
	 FEVER       & 92.6\% & 92.1\% & 91.2\% & 0.648 & 0.589 & 0.607($+$3.1\%) & 0.669 & 0.680 ($+$1.6\%) \\
	 FiQA        & 93.4\% & 91.9\% & 91.5\% & 0.239 & 0.275 & 0.276($+$0.4\%) & 0.295 & 0.296 ($+$0.3\%) \\
     ArguAna     & 92.7\% & 92.6\% & 92.6\% & 0.441 & 0.414 & 0.413($-$0.2\%) & 0.415 & 0.418 ($+$0.7\%) \\
     NQ          & 94.9\% & 93.2\% & 92.6\% & 0.310 & 0.398 & 0.402($+$1.0\%) & 0.446 & 0.442 ($-$0.9\%) \\
	 SciFact     & 91.5\% & 93.2\% & 92.8\% & 0.620 & 0.478 & 0.476($-$0.4\%) & 0.507 & 0.502 ($-$1.0\%) \\
	 SCIDOCS     & 92.2\% & 94.4\% & 93.8\% & 0.156 & 0.108 & 0.108($+$0.0\%) & 0.122 & 0.124 ($+$1.6\%) \\
   Climate-FEVER & 95.7\% & 94.7\% & 94.1\% & 0.179 & 0.176 & 0.175($-$0.6\%) & 0.198 & 0.206 ($+$4.0\%) \\
	 CQADupStack & 94.8\% & 95.2\% & 94.9\% & 0.316 & 0.281 & 0.280($-$0.4\%) & 0.296 & 0.297 ($+$0.3\%) \\
    \hline
    \end{tabular}
% 	}
	\caption{
	Overall performance and label coverage (Hole rate) on tasks from BEIR. Relative improvements of \model{} over its base DR model DPR/ANCE are shown in percentages. Datasets are ordered by ANCE's Hole rates, and datasets with lower Hole rates provide more accurate evaluation.
% 	Comparing \model{} against baselines on target domain datasets. \model's improvements are relative to ANCE.
	}
	\label{tab:overall}
\end{table*}
